Spatially Coupled Quasi-Cyclic Quantum LDPC Codes

We face the following dilemma for designing low-density parity-check codes (LDPC) for quantum error correction. 1) The row weights of parity-check should be large: The minimum distances are bounded above by the minimum row weights of parity-check matrices of constituent classical codes. Small minimum distance tends to result in poor decoding performance at the error-floor region. 2) The row weights of parity-check matrices should not be large: The sum-product decoding performance at the water-fall region is degraded as the row weight increases. Recently, Kudekar et al. showed spatially-coupled (SC) LDPC codes exhibit capacity-achieving performance for classical channels. SC LDPC codes have both large row weight and capacity-achieving error-floor and water-fall performance. In this paper, we design SC LDPC-CSS (Calderbank, Shor and Steane) codes for quantum error correction over the depolarizing channels.

==> hatHC.tex <==
\begin{tabular}
{|@{}l@{}@{}l@{}@{}l@{}@{}l@{}@{}l@{}@{}l@{}@{}l@{}|@{}l@{}@{}l@{}@{}l@{}@{}l@{}@{}l@{}@{}l@{}@{}l@{}|@{}l@{}@{}l@{}@{}l@{}@{}l@{}@{}l@{}@{}l@{}@{}l@{}|@{}l@{}@{}l@{}@{}l@{}@{}l@{}@{}l@{}@{}l@{}@{}l@{}|@{}l@{}@{}l@{}@{}l@{}@{}l@{}@{}l@{}@{}l@{}@{}l@{}|@{}l@{}@{}l@{}@{}l@{}@{}l@{}@{}l@{}@{}l@{}@{}l@{}|@{}}
\hline
&\tt{1}&&&&&&&&\tt{1}&&&&&&&&&\tt{1}&&&&&&\tt{1}&&&&&&&&&&\tt{1}&&&&&&\tt{1}&\\
&&\sf{1}&&&&&&&&\tt{1}&&&&&&&&&\tt{1}&&&&&&\sf{1}&&&\tt{1}&&&&&&&&&&&&&\tt{1}\\
&&&\tt{1}&&&&&&&&\tt{1}&&&&&&&&&\sf{1}&&&&&&\tt{1}&&&\sf{1}&&&&&&\tt{1}&&&&&&\\
&&&&\tt{1}&&&&&&&&\tt{1}&&\tt{1}&&&&&&&&&&&&&\tt{1}&&&\tt{1}&&&&&&\tt{1}&&&&&\\
&&&&&\tt{1}&&&&&&&&\tt{1}&&\tt{1}&&&&&&\tt{1}&&&&&&&&&&\tt{1}&&&&&&\tt{1}&&&&\\
&&&&&&\tt{1}&\sf{1}&&&&&&&&&\tt{1}&&&&&&\tt{1}&&&&&&&&&&\tt{1}&&&&&&\sf{1}&&&\\
\tt{1}&&&&&&&&\tt{1}&&&&&&&&&\tt{1}&&&&&&\tt{1}&&&&&&&&&&\tt{1}&&&&&&\tt{1}&&\\\hline
&&&&\tt{1}&&&&\tt{1}&&&&&&&&\tt{1}&&&&&&&&&&\tt{1}&&&&&\tt{1}&&&&&&&&&&\tt{1}\\
&&&&&\tt{1}&&&&\tt{1}&&&&&&&&\tt{1}&&&&&&&&&&\tt{1}&&&&&\tt{1}&&&\tt{1}&&&&&&\\
&&&&&&\tt{1}&&&&\tt{1}&&&&&&&&\tt{1}&&&\tt{1}&&&&&&&&&&&&\tt{1}&&&\tt{1}&&&&&\\
\tt{1}&&&&&&&&&&&\tt{1}&&&&&&&&\tt{1}&&&\tt{1}&&&&&&&&&&&&\tt{1}&&&\tt{1}&&&&\\
&\tt{1}&&&&&&&&&&&\tt{1}&&&&&&&&\sf{1}&&&\tt{1}&&&&&\tt{1}&&&&&&&&&&\sf{1}&&&\\
&&\sf{1}&&&&&&&&&&&\tt{1}&\tt{1}&&&&&&&&&&\tt{1}&&&&&\sf{1}&&&&&&&&&&\tt{1}&&\\
&&&\tt{1}&&&&\sf{1}&&&&&&&&\tt{1}&&&&&&&&&&\sf{1}&&&&&\tt{1}&&&&&&&&&&\tt{1}&\\\hline
\end{tabular}



==> hatHD.tex <==
\begin{tabular}
{|@{}l@{}@{}l@{}@{}l@{}@{}l@{}@{}l@{}@{}l@{}@{}l@{}|@{}l@{}@{}l@{}@{}l@{}@{}l@{}@{}l@{}@{}l@{}@{}l@{}|@{}l@{}@{}l@{}@{}l@{}@{}l@{}@{}l@{}@{}l@{}@{}l@{}|@{}l@{}@{}l@{}@{}l@{}@{}l@{}@{}l@{}@{}l@{}@{}l@{}|@{}l@{}@{}l@{}@{}l@{}@{}l@{}@{}l@{}@{}l@{}@{}l@{}|@{}l@{}@{}l@{}@{}l@{}@{}l@{}@{}l@{}@{}l@{}@{}l@{}|@{}}
\hline
&&&&\tt{1}&&&&&\tt{1}&&&&&&\tt{1}&&&&&&&&&&&&\tt{1}&&&&\tt{1}&&&&&&&&&\tt{1}&\\
&&&&&\tt{1}&&&&&\tt{1}&&&&&&\tt{1}&&&&&\tt{1}&&&&&&&&&&&\tt{1}&&&&&&&&&\tt{1}\\
&&&&&&\tt{1}&&&&&\tt{1}&&&&&&\tt{1}&&&&&\tt{1}&&&&&&&&&&&\tt{1}&&\tt{1}&&&&&&\\
\tt{1}&&&&&&&&&&&&\tt{1}&&&&&&\tt{1}&&&&&\tt{1}&&&&&&&&&&&\tt{1}&&\tt{1}&&&&&\\
&\tt{1}&&&&&&&&&&&&\tt{1}&&&&&&\tt{1}&&&&&\tt{1}&&&&\tt{1}&&&&&&&&&\tt{1}&&&&\\
&&\sf{1}&&&&&\sf{1}&&&&&&&&&&&&&\sf{1}&&&&&\sf{1}&&&&\sf{1}&&&&&&&&&\sf{1}&&&\\
&&&\tt{1}&&&&&\tt{1}&&&&&&\tt{1}&&&&&&&&&&&&\tt{1}&&&&\tt{1}&&&&&&&&&\tt{1}&&\\\hline
&\tt{1}&&&&&&&&&&\tt{1}&&&&&\tt{1}&&&&&&&&&&\tt{1}&&&&&&&&\tt{1}&&&&\tt{1}&&&\\
&&\tt{1}&&&&&&&&&&\tt{1}&&&&&\tt{1}&&&&&&&&&&\tt{1}&\tt{1}&&&&&&&&&&&\tt{1}&&\\
&&&\tt{1}&&&&&&&&&&\tt{1}&&&&&\tt{1}&&&\tt{1}&&&&&&&&\tt{1}&&&&&&&&&&&\tt{1}&\\
&&&&\tt{1}&&&\tt{1}&&&&&&&&&&&&\tt{1}&&&\tt{1}&&&&&&&&\tt{1}&&&&&&&&&&&\tt{1}\\
&&&&&\tt{1}&&&\tt{1}&&&&&&&&&&&&\tt{1}&&&\tt{1}&&&&&&&&\tt{1}&&&&\tt{1}&&&&&&\\
&&&&&&\tt{1}&&&\tt{1}&&&&&\tt{1}&&&&&&&&&&\tt{1}&&&&&&&&\tt{1}&&&&\tt{1}&&&&&\\
\tt{1}&&&&&&&&&&\tt{1}&&&&&\tt{1}&&&&&&&&&&\tt{1}&&&&&&&&\tt{1}&&&&\tt{1}&&&&\\\hline
\end{tabular}

